Protecting Public OSN Posts from Unintended Access

The design of secure and usable access schemes to personal data represent a major challenge of online social networks (OSNs). State of the art requires prior interaction to grant access. Sharing with users who are not subscribed or previously have not been accepted as contacts in any case is only possible via public posts, which can easily be abused by automatic harvesting for user profiling, targeted spear-phishing, or spamming. Moreover, users are restricted to the access rules defined by the provider, which may be overly restrictive, cumbersome to define, or insufficiently fine-grained. We suggest a complementary approach that can be easily deployed in addition to existing access control schemes, does not require any interaction, and includes even public, unsubscribed users. It exploits the fact that different social circles of a user share different experiences and hence encrypts arbitrary posts. Hence arbitrary posts are encrypted, such that only users with sufficient knowledge about the owner can decrypt. Assembling only well-established cryptographic primitives, we prove that the security of our scheme is determined by the entropy of the required knowledge. We consequently analyze the efficiency of an informed dictionary attack and assess the entropy to be on par with common passwords. A fully functional implementation is used for performance evaluations, and available for download on the Web.

==> proof.tex <==
\section{Proof of Theorem \ref{theo:main}}\label{app:proof}
 $\adv$ knows the encrypted post $c$, the encrypted shares $c_1,...,c_\n$, and the attribute descriptions $(d_1,\ldots,d_\n)$. 
 Let $E_{mk}$ denote the event that during the attack, the attacker made a query to the block cipher using the correct key. 
In the ideal cipher model, $c$ is equally likely to be an encryption of $p_0$ and $p_1$ if $\neg E_{mk}$. 
Hence 
\begin{eqnarray*}
\mathrm{Adv}_\adv&=&\pr{b=b^*}-1/2\\
&=&\pr{b=b^*\vert E_{mk}}\cdot\pr{E_{mk}} \\
&+& \pr{b=b^*\vert \neg E_{mk}}\cdot\pr{\neg E_{mk}}-1/2\\
&\leq &1\cdot \pr{E_{mk}}+1/2\cdot 1-1/2=\pr{E_{mk}}.
\end{eqnarray*}
Thus, the advantage of $\adv$ is equivalent to the probability $\pr{E_{mk}}$ of deriving the master key $\key$.
Let $s_1,\ldots,s_n$ denote the shares, which encode the key $\key$. Let $E_s$ denote the event that the attacker successfully reconstructed at least $t$ from these $n$ shares. Then it holds
\begin{align*}
\pr{E_{mk}}&=\pr{E_{mk}\vert E_s}\cdot \pr{E_s}+\pr{E_{mk}\vert \neg E_s}\cdot \pr{\neg E_s} \\
&\leq  Pr[E_s]+q/|\K|
%
%Pr[E_{mk}]=&Pr[E_{mk}\vert E_s]\cdot Pr[E_s]+\\
%&&Pr[E_{mk}\vert \neg E_s]\cdot \neg Pr[E_s]\\
%&\leq &1\cdot Pr[E_s]+q/|\K|.
\end{align*}
The second term follows from the fact that $\pr{E_{mk}\vert \neg E_s}\leq q/|\K|$. The reason is that if the attacker did not recover sufficient shares, it follows from the information theoretic security of the secret sharing scheme that the attacker cannot derive any information about $\key$, which he did not know before. Thus, the only remaining option in this case is to coincidently query the block cipher with the correct key. This is successful with probability at most 
$q/|\K|$. 

Next, we consider $Pr[E_s]$. Recall that the attacker only knows the encryption of the shares, being $c_i=\enc(H(v_i),s_i)$ for the selected attribute values $v_i$. Let $h_i:=H(v_i)$ denote their hash values. We denote by $E_h$ the event that the attacker correctly identified at least $t$ hash values $h_i$. It follows that 
\begin{eqnarray*}
\pr{E_s}&=&\pr{E_s\vert E_h}\cdot \pr{E_h}+\pr{E_s\vert \neg E_h}\cdot \pr{\neg E_h} \\
&\leq & 1\cdot \pr{E_h}+q/|\K|.
\end{eqnarray*}
The rationale behind the second term is similar to above: if an attacker does not know all keys which have been used to encrypt the shares, the best he can do is to guess the remaining ones.

Finally, an upper bound for $Pr[E_h]$ is derived. Let $E_v$ denote the event that the attacker identified at least $t$ values $v_i$ correctly. Using the same line of arguments, it follows that 
\begin{equation*}
\pr{E_h}\leq \pr{E_v}+q/|\K|.
\end{equation*}
Assembling all results yields the claim.\qed
%\begin{equation}
%Pr[A\ succeeds]\leq 1/2+\frac{3q}{|\mathcal{K}|}+Pr[E_v]
%\end{equation}
%Assuming that the block cipher, the hash function, and the secret sharing scheme are secure and the key space is sufficiently big, the dominating part of the success probability is given by $Pr[E_v]$, the probability to correctly guess at least $t$ values.

==> screenshots.tex <==
\section{Screenshots}
\label{app:screen}

\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{../images/post.png}
\caption{A protected note, the attributes, and the accessed content displayed by the extension}
\label{fig:post}
\end{figure}

Figure \ref{fig:post} gives an example of what an encrypted note within Facebook looks like,
together with the attributes used for protection, and the real content as displayed by the
Firefox extension after entering the correct values.

Figure \ref{fig:manager}, \ref{fig:encrypt}, and \ref{fig:decrypt} show the
dialogs for defining attributes, creating new protected notes and accessing
protected notes.
As can be seen in Figure \ref{fig:manager}, new attributes are defined by
giving a description and a value. Rather than the option 'Create Pair' in the
drop-down menu, one can also choose an old attribute for changing or deleting.
Decoupling the definition of the attributes from the actual
protection of individual posts allows easy reuse and recombination of attributes.
For each newly created note, the user first chooses a title and then enters the message,
as displayed in Figure \ref{fig:encrypt}. The number of attributes is implicitly set by the
 subset of attributes the user selects from the set defined in
the information manager before. It remains to set the threshold before creating the note.
By default, it is set to the number of attributes minus one.
In contrast, the dialog for decrypting a note (Figure \ref{fig:decrypt}) allows a user to choose the note by title
(Uni Mannheim in the example). Then fields are provided for the user to enter the
attribute values given the attribute descriptions. The number of values needed to access
the note is displayed below the title of the note. When a sufficient number of attribute values is entered correctly,
the message is displayed in the respective field, otherwise a seemingly random character string resulting
from the decryption with the incorrect key is returned.
\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{../images/informationManager.PNG}
\caption{Dialog for managing attributes}
\label{fig:manager}
\end{figure}
%
\begin{figure}
\centering
%\begin{minipage}{0.495\linewidth}
\includegraphics[width=0.95\linewidth]{../images/createNote.PNG}
\caption{Dialog for protecting a note}
\label{fig:encrypt}
%\end{minipage}
\end{figure}
%\hfill
\begin{figure}
%\begin{minipage}{0.495\linewidth}
\includegraphics[width=0.95\linewidth]{../images/decryptNote.PNG}
\caption{Dialog for accessing a note}
\label{fig:decrypt}
%\end{minipage}
%\vspace{-10em}
\end{figure}






  



